Particle Flow Gaussian Particle Filter

State estimation in non-linear models is performed by tracking the posterior distribution recursively. A plethora of algorithms have been proposed for this task. Among them, the Gaussian particle filter uses a weighted set of particles to construct a Gaussian approximation to the posterior. In this paper, we propose to use invertible particle flow methods, derived under the Gaussian boundary conditions for a flow equation, to generate a proposal distribution close to the posterior. The resultant particle flow Gaussian particle filter (PFGPF) algorithm retains the asymptotic properties of Gaussian particle filters, with the potential for improved state estimation performance in high dimensional spaces. We compare the performance of PFGPF with the particle flow filters and particle flow particle filters in two challenging numerical simulation examples.

==> bib_file.tex <==
@inproceedings{gordon1993novel,
  title={Novel approach to nonlinear/non-{G}aussian {B}ayesian state estimation},
  author={N. Gordon and D. Salmond and A. Smith},
  booktitle={IEE Proc. F Radar Signal Process.},
  volume={140},
  number={2},
  pages={107--113},
  year={1993},
  month={Apr}
}

@ARTICLE{kotecha2003GaussianSum,
author={J. H. Kotecha and  P. M. Djuric},
journal={IEEE Trans. Signal Process.},   title={Gaussian sum particle filtering},
year={2003},
month={Oct},
volume={51},
number={10},
pages={2602--2612}
}

@article{li2019,
  title={Invertible particle-flow-based sequential {MCMC} with extension to {Gaussian} mixture noise models},
  author={Y. Li and S. Pal and M. J. Coates},
  journal={IEEE Trans. Signal Process.},
  volume={67},
  number={9},
  pages={2499--2512},
  year={2019},
  month={May}
}

@incollection{bickel2008sharp,
  title={Sharp failure rates for the bootstrap particle filter in high dimensions},
  author={P. Bickel and B. Li and T. Bengtsson},
  booktitle={Pushing the limits of contemporary statistics: Contributions in honor of Jayanta K. Ghosh},
  publisher={Institute of Mathematical Statist.},
  address={Beachwood, OH, USA},
  pages={318--329},
  year={2008}
  }
  
 @incollection{bengtsson2008curse,
  title={Curse-of-dimensionality revisited: {C}ollapse of the particle filter in very large scale systems},
  author={T. Bengtsson and P. Bickel and B. Li},
  booktitle={Probability and statistics: Essays in honor of David A. Freedman},
  publisher={Institute of Mathematical Statist.},
  address={Beachwood, OH, USA},
  pages={316--334},
  year={2008}
}

@article{snyder2008obstacles,
  title={Obstacles to high-dimensional particle filtering},
  author={C. Snyder and T. Bengtsson and P. Bickel and J. Anderson},
  journal={Mon. Weather Rev.},
  volume={136},
  number={12},
  pages={4629--4640},
  year={2008},
  month={Dec}
}

@article{arulampalam2002tutorial,
  title={A tutorial on particle filters for online nonlinear/non-{G}aussian {B}ayesian tracking},
  author={M.S. Arulampalam and S. Maskell and N. Gordon and T. Clapp},
  journal={IEEE Trans. Signal Process.},
  volume={50},
  number={2},
  pages={174--188},
  year={2002},
  month={Feb}
 }
  
 @article{pitt1999filtering,
  title={Filtering via simulation: {A}uxiliary particle filters},
  author={M. Pitt and N. Shephard},
  journal={J Ameri. Statist. Assoc.},
  volume={94},
  number={446},
  pages={590--599},
  year={1999},
  month={Jun}
  }
  
  @inproceedings{doucet2000s,
  title={{Rao-Blackwellised} particle filtering for dynamic {B}ayesian networks},
  author={A. Doucet and N. d. Freitas and K. P. Murphy and S. J. Russell},
  booktitle={Proc. Conf. Uncertainty Artif. Intell.},
  address={San Francisco, CA, USA},
  pages={176},
  year={2000}
  }
  
 @article{berzuini1997dynamic,
  title={Dynamic conditional independence models and {Markov chain Monte Carlo} methods},
  author={C. Berzuini and N. G. Best and W. R. Gilks and C. Larizza},
  journal={J. Amer. Statist. Assoc.},
  volume={92},
  number={440},
  pages={1403--1412},
  year={1997},
}

@article{gilks2001following,
  title={Following a moving target — {Monte Carlo} inference for dynamic {Bayesian} models},
  author={W. R. Gilks and C. Berzuini},
  journal={J. Roy. Statist. Soc. B,},
  volume={63},
  number={1},
  pages={127--146},
  year={2001},
  month={Jan}
}

@incollection{godsill2001improvement,
  title={Improvement strategies for {Monte Carlo} particle filters},
  author={S. Godsill and T. Clapp},
  booktitle={Sequential Monte Carlo methods in practice},
  address={New York, NY, USA},
  pages={139--158},
  year={2001}
}
  
 @incollection{musso2001improving,
  title={Improving regularised particle filters},
  author={C. Musso and N. Oudjane and F. Le Gland},
  booktitle={Sequential Monte Carlo methods in practice},
  address={New York, NY, USA},
  pages={247--271},
  year={2001}
}

@article{golightly2006bayesian,
  title={Bayesian sequential inference for nonlinear multivariate diffusions},
  author={A. Golightly and D. Wilkinson},
  journal={Statist. Comput.},
  volume={16},
  number={4},
  pages={323--338},
  year={2006},
  month={Dec}
}

@article{maroulas2012improved,
  title={Improved particle filters for multi-target tracking},
  author={V. Maroulas and P. Stinis},
  journal={J. Comput. Phys.},
  volume={231},
  number={2},
  pages={602--611},
  year={2012},
  month={Jan}
}

@inproceedings{kang2014drift,
  title={Drift homotopy particle filter for non-{Gaussian} multi-target tracking},
  author={K. Kang and V. Maroulas and I. D. Schizas},
  booktitle={Proc. Int. Conf. Inf. Fusion},
  address={Salamanca, Spain},
  pages={1--7},
  year={2014}
}

@article{brockwell2010sequentially,
  title={Sequentially interacting {Markov chain Monte Carlo} methods},
  author={A. Brockwell and P. D. Moral and A. Doucet},
  journal={Ann. Statist.},
  volume={38},
  number={6},
  pages={3387--3411},
  year={2010},
  month={Dec}
}

@article{septier2015langevin,
  title={Langevin and {Hamiltonian} based sequential {MCMC} for efficient {Bayesian} filtering in high-dimensional spaces},
  author={F. Septier and G. W. Peters},
  journal={IEEE J. Sel. Topics Signal Process.},
  volume={10},
  number={2},
  pages={312--327},
  year={2016},
  month={March}
}

@article{article,
title = {Gaussian Particle Filtering},
author = {J. Kotecha and P. Djuric},
journal = {IEEE Trans. Signal Process.},
year = {2003},
month = {Nov},
pages = {2592 - 2601},
volume = {51},
}

@inproceedings{daum2007nonlinear,
  title={Nonlinear filters with log-homotopy},
  author={F. Daum and J. Huang},
  booktitle={Proc. SPIE},
  volume={6699},
  pages={423--437},
  year={2007},
  month={Sep.}
}

@inproceedings{daum2008particle,
  title={Particle flow for nonlinear filters with log-homotopy},
  author={E. Daum and J. Huang},
  booktitle={Proc. SPIE},
  volume={6969},
  pages={696918},
  year={2008},
  month={Apr}
}

@inproceedings{daum2009gradient,
  title={Gradient estimation for particle flow induced by log-homotopy for nonlinear filters},
  author={F. Daum and J. Huang and A. Noushin and M. Krichman},
  booktitle={Proc. SPIE },
  volume={7336},
  pages={65--75},
  year={2009},
  month={Apr},
  organization={SPIE}
}

@inproceedings{daum2010exact,
  title={Exact particle flow for nonlinear filters},
  author={F. Daum and J. Huang and A. Noushin},
  booktitle={Proc. SPIE},
  volume={7697},
  pages={769704},
  year={2010},
  month={Apr}
}

@inproceedings{daum2013particle,
  title={Particle flow with non-zero diffusion for nonlinear filters},
  author={F. Daum and J. Huang},
  booktitle={Proc. SPIE},
  volume={8745},
  pages={87450P},
  year={2013},
  month={May}
}

@inproceedings{daum2014seven,
  title={Seven dubious methods to mitigate stiffness in particle flow with non-zero diffusion for nonlinear filters, {Bayesian} decisions, and transport},
  author={F. Daum and J. Huang},
  booktitle={Proc. SPIE},
  volume={9092},
  pages={72--82},
  year={2014},
  month={May}
}

@inproceedings{li2015particle,
  title={Particle flow auxiliary particle filter},
  author={Y. Li and L. Zhao and M. J. Coates},
  booktitle={Proc. Comput. Adv. Multi-Sensor Adapt. Process.},
  pages={157--160},
  year={2015},
  month={Dec}
}

@inproceedings{7472424,
  author={Y. Li and L. Zhao and M. J. Coates},
  booktitle={Proc. Int. Conf. Acoust. Speech Signal Process.}, 
  title={Particle flow for particle filtering}, 
  year={2016},
  pages={3979-3983},
 }
 
 @inproceedings{ding2012implementation,
  title={Implementation of the {Daum-Huang} exact-flow particle filter},
  author={T. Ding and M. J. Coates},
  booktitle={Proc. IEEE Statist. Signal Process. Workshop},
  pages={257--260},
  year={2012}
}

@article{li2017particle,
  title={Particle filtering with invertible particle flow},
  author={Y. Li and M. J. Coates},
  journal={IEEE Trans. Signal Process.},
  volume={65},
  number={15},
  pages={4102--4116},
  year={2017},
  month={Aug}
}

@book{warner1983foundations,
  title={Foundations of differentiable manifolds and {Lie} groups},
  author={F. W. Warner},
  volume={94},
  year={1983},
  publisher={Springer Science \& Business Media}
}

@inproceedings{hlinka2011distributed,
  title={Distributed {Gaussian} particle filtering using likelihood consensus},
  author={O. Hlinka and O. Slu{\v{c}}iak and F. Hlawatsch and P. M. Djuri{\'c} and M. Rupp},
  booktitle={Proc. Int. Conf. Acoust. Speech Signal Process.},
  address={Prague, Czech Republic},
  pages={3756--3759},
  year={2011},
  month={May}
}

@article{schuhmacher2008consistent,
  title={A consistent metric for performance evaluation of multi-object filters},
  author={D. Schuhmacher and B. T. Vo and B. N. Vo},
  journal={IEEE Trans. Signal Process.},
  volume={56},
  number={8},
  pages={3447--3457},
  year={2008},
  month={Aug}
}

@article{zhu2010generalized,
  title={A generalized asymmetric {S}tudent-t distribution with application to financial econometrics},
  author={D. Zhu and J. W. Galbraith},
  journal={Journal of Econometrics},
  volume={157},
  number={2},
  pages={297--305},
  year={2010},
  month={Aug}
}

@inproceedings{khan2015improvements,
  title={Improvements in the implementation of log-homotopy based particle flow filters},
  author={M. A. Khan and M. Ulmke},
  booktitle={Proc. Int. Conf. Inf. Fusion},
  pages={74--81},
  year={2015}
}

@inproceedings{pal2019particle,
  title={Particle flow particle filter using {G}romov's method},
  author={S. Pal and M. J. Coates},
  booktitle={Proc. Comput. Adv. Multi-Sensor Adapt. Process.},
  pages={634--638},
  year={2019},
  month={Dec}
}

@inproceedings{daum2010exact1,
  title={Exact particle flow for nonlinear filters: seventeen dubious solutions to a first order linear underdetermined {PDE}},
  author={F. Daum and J. Huang},
  booktitle={Proc. Asilomar Conf. Signals, Syst. Comput},
  pages={64--71},
  year={2010},
  month={Nov}
}

@article{lee1994extended,
  title={Extended {Kalman} filter based nonlinear model predictive control},
  author={J. H. Lee and N. L. Ricker},
  journal={Industrial \& Engineering Chemistry Research},
  volume={33},
  number={6},
  pages={1530--1541},
  year={1994},
  month={Jun}
}

@article{wan2001unscented,
  title={The unscented {Kalman} filter},
  author={E. A. Wan and R. Van Der Merwe and S. Haykin},
  journal={Kalman filtering and neural networks},
  volume={5},
  number={2007},
  pages={221--280},
  year={2001},
}

@article{evensen2003ensemble,
  title={The ensemble {K}alman filter: Theoretical formulation and practical implementation},
  author={G. Evensen},
  journal={Ocean Dyn.},
  volume={53},
  number={4},
  pages={343--367},
  year={2003}
}

@inproceedings{julier1997new,
  title={New extension of the {Kalman} filter to nonlinear systems},
  author={Julier, Simon J and Uhlmann, Jeffrey K},
  booktitle={Proc. SPIE},
  volume={3068},
  pages={182--193},
  year={1997},
  month={Apr}
}
